FourierHandFlow: Neural 4D Hand Representation Using Fourier Query Flow

Recent 4D shape representations model continuous temporal evolution of implicit shapes by (1) learning query flows without leveraging shape and articulation priors or (2) decoding shape occupancies separately for each time value. Thus, they do not effectively capture implicit correspondences between articulated shapes or regularize jittery temporal deformations. In this work, we present FourierHandFlow, which is a spatio-temporally continuous representation for human hands that combines a 3D occupancy field with articulation-aware query flows represented as Fourier series. Given an input RGB sequence, we aim to learn a fixed number of Fourier coefficients for each query flow to guarantee smooth and continuous temporal shape dynamics. To effectively model spatio-temporal deformations of articulated hands, we compose our 4D representation based on two types of Fourier query flow: (1) pose flow that models query dynamics influenced by hand articulation changes via implicit linear blend skinning and (2) shape flow that models query-wise displacement flow. In the experiments, our method achieves state-of-the-art results on video-based 4D reconstruction while being computationally more efficient than the existing 3D/4D implicit shape representations. We additionally show our results on motion inter- and extrapolation and texture transfer using the learned correspondences of implicit shapes. To the best of our knowledge, FourierHandFlow is the first neural 4D continuous hand representation learned from RGB videos. The code will be publicly accessible.

==> sections/3_preliminaries.tex <==
\section{Preliminaries}

\subsection{Linear Blend Skinning (LBS)}
\label{subsec:lbs}

We first review linear blend skinning (LBS), which is a widely-used technique to deform a shape with underlying skeletal structures. It is originally proposed for deforming a \emph{mesh} according to rigid bone transformations~\cite{SMPL:2015, MANO:SIGGRAPHASIA:2017}. Given a mesh with a set of $N$ initial vertex positions $\{\hat{\mathbf{v}}^{(i)}\}_{i=1}^N$ and rigid transformation matrices of $B$ bones $\{\mathbf{T}_b\}_{b=1}^{B}$, the deformed vertex positions $\{\mathbf{v}^{(i)}\}_{i=1}^N$ are computed as:

\vspace{-0.5\baselineskip}
\begin{equation}
\mathbf{v}^{(i)} = \sum^{B}_{b=1} \, \mathbf{w}_{b}^{(i)} \, \mathbf{T}_{b} \, \hat{\mathbf{v}}^{(i)}, \:\:\: \forall i = 1, ..., N,
\label{eq:mesh_lbs}
\end{equation}

\noindent where $\mathbf{w}^{(i)} \in [0, 1]^B$ is a skinning weight vector for $\hat{\mathbf{v}}^{(i)}$ \emph{s.t.} $\sum_{b=1}^{B}\mathbf{w}^{(i)}_{b} = 1$. Each entry $\mathbf{w}^{(i)}_b$ represents the amount of influence that $\mathbf{T}_b$ has on the deformed position of $i$-th vertex.

Recently, neural implicit shape representations in 3D domain~\cite{mihajlovic2021leap,saito2021scanimate} have also adopted LBS for articulated shape modeling. Since LBS weights should be implicitly defined given an arbitrary 3D query position, they use a neural network $w(\cdot): \mathbb{R}^3 \rightarrow [0, 1]^B$ to learn the mapping from an input query $\mathbf{p} \in \mathbb{R}^{3}$ to the corresponding skinning weight vector $\mathbf{w}^{\mathbf{p}} \in [0, 1]^{B}$. Analogous to Eq. (\ref{eq:mesh_lbs}), the deformed query position is computed by applying the average of the transformations $\{\mathbf{T}_{b}\}_{b=1}^{B}$ weighted by $\mathbf{w}^{\mathbf{p}}$. 

%Our method also utilizes an implicit LBS weight field to model query flow induced by the change of hand pose.

\subsection{Learning for Canonical Hand Occupancy and Implicit LBS Weights}
\label{subsec:pre_learning}

Our 4D implicit hand representation learns query flows (\emph{i.e.}, trajectories) that are continuous in both space and time. Similar to Occupancy Flow~\cite{niemeyer2019occupancy}, we assign occupancy values to the queries sampled in the reference coordinate system and then propagate the occupancies along the learned query flows to enable 4D reconstruction. While Occupancy Flow~\cite{niemeyer2019occupancy} considers a coordinate system at $t=0$ as the reference coordinate system separately for each sequence, we use a canonical hand shape system for all sequences and transfer hand canonical occupancies along the time axis to perform 4D reconstruction. This was inspired by recent 3D implicit representations of human bodies and hands~\cite{mihajlovic2021leap,karunratanakul2021skeleton,lee2023im2hands} that shows learning an occupancy field and an LBS field in the canonical system is more robust than learning them directly in the posed system. 
% that addresses learning an occupancy field and an LBS field in the canonical system is more robust than learning them directly in the posed system. 

Our occupancy and LBS weight fields are formally defined as $o(\cdot): \mathbb{R}^{3} \rightarrow [0, 1]$ and $w(\cdot): \mathbb{R}^{3} \rightarrow [0, 1]^{B}$, which maps a query point $\mathbf{p} \in \mathbb{R}^{3}$ in the canonical hand space to an occupancy probability $o(\mathbf{p}) \in [0, 1]$ and LBS weights $w(\mathbf{p}) \in [0, 1]^{B}$, respectively. They are learned prior to learning query flows using a modified architecture of LEAP~\cite{mihajlovic2021leap}. For more details, we kindly refer the reader to the supplementary section. 

% canonical hand occupancy field and lbs field using any learning mechanism is fine. <= 이걸 넣어야 할 듯

\textcolor{blue}{Jihyun: need to organize the notations...}

%Once the hand occupancy and LBS weight fields in our canonical reference system are obtained, they are globally used for training and inference for our Fourier-based flow network, which will be discussed in the following section.

% mention that manual template can be also used. ?


==> tables/rep_power.tex <==
\begin{table}[h]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Representation power (least priority).}}
\label{table:rep_power}

\begin{tabularx}{\columnwidth}{>{\centering}m{2.4cm}|>{\centering}m{4.8cm}|Y|Y}
\toprule
Category & Method & IoU \footnotesize{(\%)} $\uparrow$ & CD \footnotesize{(mm)} $\downarrow$ \\
\midrule
3D Implicit & Im2Hands~\cite{lee2023im2hands} & ? & ? \\
\midrule
\multirow{3}{*}{4D Implicit} & Occupancy Flow~\cite{niemeyer2019occupancy} & ? & ? \\ 
& LoRD$^\dag$~\cite{jiang2022lord} & ? & ? \\
& \textsc{FourierHandFlow} (Ours) & ? & ? \\
\bottomrule
\end{tabularx}
}
\end{table}
